GEM: Group Enhanced Model for Learning Dynamical Control Systems

Learning the dynamics of a physical system wherein an autonomous agent operates is an important task. Often these systems present apparent geometric structures. For instance, the trajectories of a robotic manipulator can be broken down into a collection of its transitional and rotational motions, fully characterized by the corresponding Lie groups and Lie algebras. In this work, we take advantage of these structures to build effective dynamical models that are amenable to sample-based learning. We hypothesize that learning the dynamics on a Lie algebra vector space is more effective than learning a direct state transition model. To verify this hypothesis, we introduce the Group Enhanced Model (GEM). GEMs significantly outperform conventional transition models on tasks of long-term prediction, planning, and model-based reinforcement learning across a diverse suite of standard continuous-control environments, including Walker, Hopper, Reacher, Half-Cheetah, Inverted Pendulums, Ant, and Humanoid. Furthermore, plugging GEM into existing state of the art systems enhances their performance, which we demonstrate on the PETS system. This work sheds light on a connection between learning of dynamics and Lie group properties, which opens doors for new research directions and practical applications along this direction. Our code is publicly available at: https://tinyurl.com/GEMMBRL.

==> sections/Abstract_params.tex <==
\section{Parameters of training}\label{sec:AppendixTechDetails}

==> sections/GEM.tex <==
\begin{tikzpicture}[scale=.65, transform shape, every node/.style={thick,circle,inner sep=0pt},every text node part/.style={align=center}]

    \node[opacity=1.0] (n210) at (+4.2, +2.25-3.85) {{\bf GEM: Group Enhanced Model}};

    \node[opacity=1.0, circle] (n37) at (+9.75, +0.5-4) {$\mathbf{\hat{s}_{t+1}}$};

      \node[regular polygon,regular polygon sides=9,draw=black,inner sep=0pt,scale=0.75] (n35) at (+8.6, +0.5-4) {$\mathbf{G_{t+1}}$};
   
    %  \node[opacity=1.0] (n36) at (+7.2, +0.5-5.1) {$\mathbf{\hat{G}_{t+1}}(\theta)\doteq\exp(\sum_i\hat{\alpha}_{i,t}(\theta)\cdot E_i)\circ G_t$};
     \node[opacity=1.0] (n36) at (+7.2, +0.5-5.1) {$\mathbf{\hat{G}_{t+1}} = \exp(\mathbf{\hat{g}_{t}})\circ G_t$ by \eqref{eq:LieDynamics}};
    
     \node[circle, draw=black!80, minimum size=1cm] (n34) at (+7.2, +0.5-4) {$\mathbf{\circ}$};
    
    \node[circle, draw=black!80, minimum size=1cm] (n33) at (+5.7, +0.5-4) {{\bf EXP}};
    
    % \node[rectangle, fill=Red!40, minimum size=1cm](n32) at (+5.25, +0.5-4) {$\mathbf{g_{t}}\in\mathfrak{g}$};  
    \node[rectangle, draw=black, minimum size=1cm](n32) at (+4.2, +0.5-4) {$\mathbf{\hat{g}_{t}}$};  
    % \mathbf{g_{t}}\doteq\sum_i\alpha_{t,i}\cdot E_i$
    \node[opacity=1.0] (n31) at (+4, +0.5-3.15) {{ $\mathbf{\hat{g}_t}=\sum_{i}\hat{\alpha}_{i,t}\cdot E_i$}  by \eqref{eq:algebraelement}};
    
    % \node[rectangle, minimum size=0.74cm, fill=NavyBlue!60] (n30) at (+4, +0.5-4) {$ $\\$E_1$\\$E_2$\\$\cdots$\\$E_k$\\$ $};
     
    \node[circle, opacity=1.0] (n29) at (+3, +0.5-4) {$\mathbf{\hat{\alpha}_{t}}$};
    
    \node[regular polygon,regular polygon sides=9,draw=black] (n28) at (-1, +1.0-4) {$\mathbf{G_{t}}$};
    
    \node[circle, opacity=1.0] (n28s) at (-2, +1.0-4) {$\mathbf{s_{t}}$};
    
    \node[circle, opacity=1.0] (n27) at (-1, +0.0-4) {$\mathbf{a_{t}}$};
    \node[circle,  fill=Red!30] (n26) at (2, +0.5-4)    {$\theta$};
    \node[circle,  fill=Red!30] (n25) at (1, +1.5-4)    {$\theta$};
    \node[circle,  fill=Red!30] (n24) at (1, +0.5-4)    {$\theta$};
    \node[circle,  fill=Red!30] (n23) at (1, -0.5-4)    {$\theta$};
    \node[circle,  fill=Red!30] (n22) at (0,  1-4)      {$\theta$};
    \node[circle,  fill=Red!30] (n21) at (0,  0-4)      {$\theta$};
    \foreach \from/\to in { n21/n23, n21/n24, 
                            n21/n25, n22/n23, 
                            n22/n24, n22/n25,
                            n23/n26, n24/n26, 
                            n25/n26, n27/n21, 
                            n28/n22, n26/n29, 
                            n29/n32, 
                            n32/n33, n33/n34,
                            n28s/n28, n34/n35,       n35/n37}
\draw [->] (\from) -- (\to);
\draw [->,rounded corners] (n28.north) |- ++(7.6,0.5) -| (n34.north);
\begin{pgfonlayer}{background}
        \path (n28.west |- n28.north)+(-0.95,+1.5) node (a) {};
        \path (n28.east -| n28.east)+(+10.85,-4.7) node (c) {};
        \path[fill=gray!1,fill opacity=1.0,rounded corners, draw=black!10, dashed] (a) rectangle (c);           
\end{pgfonlayer}

\begin{pgfonlayer}{background}
        \path (n22.west |- n22.north)+(-0.275,+0.5) node (a) {};
        \path (n22.east -| n22.east)+(+2.0,-1.7) node (c) {};
        \path[fill=Gray!50,fill opacity=0.2,rounded corners, draw=black!10, dashed] (a) rectangle (c);           
\end{pgfonlayer}

% \node[circle, opacity=1.0] (NN) at (1.75, +0.5-6) {$\mathcal{NN}$}

% \node[circle, opacity=1.0] (l1) at (-1.6, +1.0-6) {Legend:};
\node (l1) at (+0.5, +1.0-7.2) {{

    {\begin{varwidth}{\linewidth}
    \hspace{0.35cm}{\large Legend:
    \begin{itemize}
           \item $\alpha_t$ - Lie algebra coefficients
        % \vspace{-0.25cm}
        \item $\hat{g}_t$ - Lie algebra element
        % \vspace{-0.25cm}
        \item $G_t, \hat{G}_{t+1}$ -  Lie group elements
    \end{itemize}}\end{varwidth}}
}};
\node (l2) at (+6.5, +1.0-7.2) {{

    {\begin{varwidth}{\linewidth}
    \hspace{0.35cm}%Legend:
    {\large \begin{itemize}
      \item $\{E_1, E_2, \dots\}$ - Lie algebra basis
        % \vspace{-0.25cm}
        \item $\mathbf{\circ}$ - Lie group operation
        % \vspace{-0.25cm}
        \item $\mathbf{EXP}$ - exponential map: $\mathfrak{g}\rightarrow \mathfrak{G}$ 
    \end{itemize}}\end{varwidth}}
}};
\end{tikzpicture}

==> sections/abstract_cmt_original.tex <==
Artificial agents often operate in environments where the geometric structures of the underlying physical systems are known. For instance, the trajectories of a robotic manipulator can be broken down into a collection of its transitional and rotational motions, fully characterized by the corresponding Lie groups and Lie algebras. In this work, we take advantage of these structures to build effective dynamical models that are amenable to experience-based learning. We hypothesize that learning the dynamics on a Lie algebra vector space is more effective than learning a direct state transition model. To verify this hypothesis, we introduce the Group Enhanced Model (GEM). GEMs significantly outperform the conventional transition models in the task of both long-term prediction and model-based reinforcement learning on a diverse suite of standard continuous-control environments, including walker, hopper, reacher, half-cheetah, inverted pendulums, ant, humanoid, etc. Our work sheds light on a connection between learning of dynamics and Lie group properties, which opens doors for new research directions and practical applications along this direction.  We make our code available at https://tinyurl.com/GEMICML.

==> sections/abstract_old.tex <==
\begin{abstract}
\PH{comment}, \WS{comment}, \LP{comment}, \ST{comment}

%In this work we take advantage of the structure \PH{structure of the env as well? Perhaps assumed already} of manifolds for sample-based learning of dynamical systems.\WS{the first sentence becomes redundant}
Learning of an accurate dynamics model is an important task, e.g. in model-based control problems. \ST{Usually in learning, the states of dynamical system are represented and treated as Euclidean vectors without a particular structure.} However, assuming the states form a manifold, we can take advantage of the manifold's rich structure to efficiently capture the underlying dynamical system via sample-based learning. In this work, we consider a scenario where the states of a dynamical system form a Lie group. The states thus evolve on the Lie group manifold according to the corresponding Lie algebra vector space. We hypothesize that learning the dynamics on this vector space is more effective than learning a direct state transition model. To test this hypothesis we introduce a special framework for neural networks with explicit Lie-algebraic priors. We verify our hypothesis on various dynamical control systems, \ST{including pendulums, reacher, walker, half-cheetah, humanoid, and other standard robotic benchmark systems}, where our method significantly outperforms the baseline of learning state transition. Our work sheds light on a connection between learning of dynamics and Lie group properties, which opens doors for new research directions and practical applications along this direction. We make our code available at: anonymous-githab-account.
\end{abstract}

%Sample-efficient learning of an accurate dynamics model is an important task, e.g. in model-based control problems. Assuming the states form a smooth manifold, we can take advantage of the manifold's rich structure to efficiently capture the underlying dynamical system via sample-based learning. 

% This document provides a basic paper template and submission guidelines.
% Abstracts must be a single paragraph, ideally between 4--6 sentences long.
% Gross violations will trigger corrections at the camera-ready phase.

% Learning a precise model of dynamics from samples is an important task. In this work we take advantage of the structure of smooth differentiable manifolds for learning precise models. Particularly, we consider state samples of dynamics as Lie group elements, evolving on the manifold according to a corresponding Lie algebra, which is a vector space. We hypothesize that learning dynamics directly on this vector space enables to achieve more precise models in comparison to the common approach for learning of dynamics from unstructured state-vector samples. We confirm our hypothesis on various dynamical control systems, where our method achieves a significantly lower (PUT NUMBER) long-term prediction error. We demonstrate the advantage of our method on several standard benchmarks for planning and reinforcement learning. Our method is realized by a new type of deep neural network architecture, (which can be seamlessly plugged into the existing system), with an explicit algebraic priors. The code is available at (PUT github-anonymous-link, which enables to reproduce the plots). This work sheds lights on the connection between statistical machine learning and Lie group structures. We defer the theoretical question on the reduction of sample complexity of learning due to incorporation of Lie-algebraic priors to the future work. We defer the theoretical questions on the reduction of sample complexity of learning due to incorporation of Lie-algebraic priors to the future work.  especially for precise modeling of complex high-dimensional dynamics,

% Also, we demonstrate the advantage of our method on several standard benchmarks for planning and reinforcement learning.

==> sections/applications.tex <==
\section{Applications}\label{sec:Applications}
\ST{why is it important for the readers to see these plots? we show already that Lie is stronger in prediction. That is important to show that the gap in performance does not close even if we continuous update the models in MBRL cycle}
To address our second main question, we set up experiments to apply the models on downstream tasks. We largely saw better long horizon prediction in the main results section for GEM, it is then important to show that this gap in performance is maintained during usage of the model for optimal control [REF].\ST{unclear what does extension to dynamics model mean?} \ST{REFS}. In Section 6.1 we discuss planning on the models without any environment observation update \ST{unclear. think as this reads a stranger. which isolation/isolation from what/whom?}. In Section 6.2, we apply a standard Model Based Reinforcement Training loop [REF] \ST{RL training loop? if it is MBRL say that, and and references} to understand the evolution of performance of the model with the number of samples trained on as well as to see its performance on long term planning with interval environment observation updates.

\subsection{Planning}
We perform planning experiments on continuous control tasks to evaluate the usefulness of the model outside of state prediction. A model with strong long horizon prediction will largely be a good model for use in planning and optimal control(REF). It is important to note in these experiment that apart from the first observation, no update from the environment is provided to the models. We do this to analyze the capabilities of the models as pure belief updates, this will put under scrutiny the strength of long horizon prediction.

\myinput{./sections/planningRewardCurves}

In Figure \eqref{fig:Planning Cumulative Reward Averaged} we see the rewards achieved from planning on trained models. Since this is planning with no update from the environment apart from the first step, the planner relies heavily on the model to select optimal actions. We see the benefits of long horizon prediction from the main results transfer to planning. GEM achieves higher rewards on average on all presented tasks. In some tasks, the baseline has largely collapse or decayed in performance, but GEM remains viable for longer. \ST{good said!}
\subsection{Reinforcement Learning}
To further evaluate the performance of the models in realistic and applicable tasks, we input the model into a Model Based Reinforcement Learning training loop [REF]. We cycle between planning and collecting data into replay buffer and training model\ST{REFs} in standard MBRL format (REF). This experiment will give us more answers on main question two and three: the performance of the models on task sets and its sample efficiency. Again, it is important to note that we only update the model with an observation from the environment every 5 steps in a trajectory. We firstly want to evaluate the strength of the model and secondly want to provide a realistic case where one many not have access to the environmental data every for every step. This could be from the expensive of fetching observations, sensors losing connection, or unreliable data being provided.\ST{<- unclear sentence. also, "we hope" does not sound good in an academic paper}

\myinput{sections/mbrPlots}

Figure \eqref{fig:MBRL Reward Averaged} shows the performance of GEM and the baselines when trained in a more standard and realistic format [REF]. We continue to see the large over performance of GEM over the baselines in rewards achieved and in sample efficiency. Under the same amount of samples collected, GEM averages four times the rewards of the baselines. Because of the lack of constant per step update, the planner relies on the model periodically to plan out policy. For this reason, the generic never lasts very long in environments that are potentially unstable (e.g. pendulum environments) due to its poor long horizon prediction ability. GEM on the other hand, last much longer in these environments.


==> sections/intro.tex.bck.2 <==
\section{Introduction}\label{sec:Intro}
Interaction between an autonomous agent and its environment is often modeled by a dynamical control system, where the current state and agent's action are mapped by a dynamics function to the next state~\citep{watter2015embed,todorov2005generalized}. When the system is unknown and complex, reliably learning the dynamical model from data samples is a notably challenging problem [REFs]. Reliable dynamical models are required in many important scenarios such as planning~\citep{schrittwieser2020mastering}, model-based reinforcing learning~\citep{moerland2020model}, system identification~\citep{nelles2020nonlinear}, environment emulation~\citep{castelletti2012data}, SimToReal [REFs], and many others. Moreover, often, a long-term horizon reliability is of an interest, which is a significantly more challenging problem as compared to a single-step models [REfs]. For this reason, avid research efforts are dedicated to enhancing the quality of sample-based methods for learning of dynamical models~\citep{brzeski2017sample, fragkiadaki2015recurrent, deisenroth2011learning} [more REFs].    

%\st{However, it is notably challenging to learn a reliable dynamics function especially in high-dimensional environments [REFs]}. 
% \ST{ADD WHY LONG TERM PREDICTION IS IMPORTANT, AND WHY A SINGLE STEP IS NOT ENOUGH. THAT IS OUR STRENGTH} 
%We overview the relevant works in Section \ref{sec:relevant}. 

% \input{sections/scheme1_v2}
% \input{sections/scheme1}

\begin{figure*}[t]
\centering
\includegraphics[scale=0.75]{./images/MAINPICTURE}
\caption{}
\end{figure*}

In general, the problem of learning a dynamical model is formulated as learning a predictive mapping from the present state and action to the future state~\citep{schrittwieser2020mastering}. Usually, the outputs and the inputs in learning of this mapping are considered and treated as general Euclidean vectors [general REEFs to learning of models] overlooking intrinsic properties within the state space of dynamical system. The later is a manifold of a particular structure ~\citep{strogatz2018nonlinear,agrachev2013control}, which can be potentially exploited for learning. Thus, a promising research direction would be to incorporate the structure of smooth manifolds to learning of reliable dynamical models.



% As shown previously, incorporating the underlying structure, i.e. the inductive bias of the state space, can greatly improve existing algorithms over various applications [REFs image recognition, classification, robotics etc]. Thus, a promising research direction would be to incorporate the structure of smooth manifolds to sample-based learning of dynamics.\WS{I am a bit confused here. This work should be filling some gap that previous work is not doing. But it seems "sample-based learning of dynamics" is too general a term to describe this gap. Also, is "sample-based learning" essentially...machine learning? i.e. learning from data?}

% \begin{figure}[t]
%   \centering
    % \includegraphics[width=0.5\textwidth]{./images/Fig1_place_holder2}
%   \caption{MDP-Lie Group-Lie Algebra-Lie Group.}\label{fig:Scheme}
% \end{figure}

% \begin{figure}[t]
%   \centering
%     \includegraphics[width=0.5\textwidth]{./images/Fig1_place_holder}
%   \caption{Scheme.}\label{fig:Scheme}
% \end{figure}

\ST{In this work, we propose a novel framework that takes advantage of the intrinsic properties of the smooth manifold for learning a dynamical models. To characterize the intrinsic properties, we follow the framework of Lie group theory. } 

To this end, we propose the \emph{Group Enhanced Models} (GEMs) that effectively learn dynamics functions over Lie group manifolds from experiences. 

Section~\ref{sec:Preliminaries} will review the relevant background of Lie group theory.


Central to GEMs is the one-to-one correspondence between elements from the manifold and those from an associated linear vector space, termed Lie Algebra. The Lie Algebra is constructed as the tangential space at the identity element of Lie group manifold. The significance of this correspondence is nicely summarized in the following paragraph by \citep{howe1983very}:
\begin{quotation}
{\it
\noindent ...The essential phenomenon of Lie theory is that one may associate in a natural way to a Lie group $\mathcal{G}$ its Lie algebra $\mathfrak{g}$. Thus for many purposes one can replace $\mathcal{G}$ with g. Since $\mathcal{G}$ is a complicated nonlinear object and $\mathfrak{g}$ is just a vector space, it is usually vastly simpler to work with $\mathfrak{g}$...} 
\end{quotation}
\begin{remark}\label{eq:Hypothesis}
Therefore, we also hypothesize that it is more efficient and effective to learn a dynamics function on the linear vector space, Lie algebra, $\mathfrak{g}$, than on the original unstructured raw state space, $\mathcal{S}$ or on the complicated Lie group $\mathfrak{G}$.
\end{remark}

 
%because the former reflects the structure of dynamics, while the later allows us only to map the present state to the future state regardless of the dynamics structure. 
\ST{Figure \eqref{fig:scheme1} shows a scheme of our method, which we describe in Section \ref{sec:Method}. tbd: CONNECT TEXT TO THE FIGURE, AND EXPLAIN WHAT CAPTION DOES NOT TELL} 

%There are several levels of knowledge of a dynamical system, ranging from model-free (full model ignorance) to model-based (full model knowledge) interactions between the agent and the environment [REFs]. 
To elaborate, in this work, assuming the dynamical model of the environment is not given, we strive on the middle ground between model-free (full model ignorance) and model-based (full model specification) to obtain an intermediate knowledge level of a dynamical system. To do so, we consider learning of dynamics on Lie algebra as a primitive geometric prior. 

When a dynamical model is not given, it needs to be captured from experience replays. An important component for experience-based learning of dynamics is the choice of priors over the dynamics models, usually coming from our understanding of the underlying physical laws. For example, the priors can be some distribution over the model parameters [REfs] or a set of differential equations with undetermined physical parameters [REfs]. Here, we consider another type of priors, which are primitive geometric motions of dynamical system. 
%
\ST{ADD A PICTURE A CAR} Primitive geometric priors describe \textit{what a dynamical system does}, which is independent from any specific physical parameters (such as friction, mass, natural frequencies, etc) or physical laws. For example, by simply observing interactions between the agents and the environments, one may understand that a car rotates and translates linearly, a robotic arm rotates around rotation axes of its joints, and a humanoid translates its center of mass while rotating its hinge joints. Such information can usually be obtained either implicitly via camera [REF orintetion detection by camera] or explicitly via hardware specifications~\citep{todorov2012mujoco} with little extra cost. In contrast, many physical states need to be measured by elaborated motion capture or sensory systems~\citep{OpenAIHand}.  \ST{WE HAVE GEOMETRIC STRUCTURE OF THE MODEL, ELABORATE ON THIS. GEOMETRIC KNOWLEDGE IS VERY CHEAP, PHYSICS IS EXPENSIVE} \WS{from To this end, we propose the \emph{Group Enhanced Models} (GEMs) to the end of this paragraph is not  clear what is the flow.}

Our main contributions are:
% \vspace{-0.5cm}
\begin{itemize}[noitemsep,topsep=0pt]
    \item We propose a novel class of deep neural network framework, the \emph{Group Enhanced Models}, to learn dynamics function on Lie algebra..
    \item We experimentally show that GEM outperforms the existing baselines on the task of \textit{long-term horizon prediction} on the standard benchmarks, including both low and high-dimensional systems such as chaotic double-pendulum, hopper, half-cheetah, humanoid, and others. 
    \item We demonstrate the advantage of GEM over various important applications of model-based reinforcement learning, planning \ST{elaborate on }, and model-based policy optimization, and others. 
\end{itemize}              
In Section \ref{sec:relevant}, we review the related prior works in comparison to GEM, emphasizing its novelty. Section~\ref{sec:Preliminaries} goes over the most relevant technical background of Lie group theory to our proposed framework. Section \ref{sec:mainresult} presents the main experimental results. Section \ref{sec:Applications} demonstrates how to apply GEM to a model-based RL application. Finally, Section \ref{sec:discussion} discusses the promising future research directions.
%aiming to extend our knowledge about the connection between the properties of smooth manifolds and sample-based learning, and propose applicative extensions of our current implementation. 










==> sections/mainresults_back.tex <==
\section{Main Results}\label{sec:mainresult}
We now evaluate our model on a standard set of continuous control dynamical systems\ST{->on a standard set of continuous control dynamical , commonly used to evaluate reinforcement learning algorithms [5 REFs <- Ref]}. They are as follows, Inverted Pendulum, Inverted Double Pendulum, Reacher, Hopper, Walker, Half Cheetah, Ant, and Humanoid. We choose these environments due to the diverse set of challenging geometries and motions incorporated in each system. [REF papers that use similar set of envs] \ST{why we chose these envs? justification} 

Section 4.1 discusses the comparison of long term prediction errors \ST{Comparison of Long Term Prediction of something like this. "overall comparison" is an empty statement.} between baseline models and GEM. Section 4.2 scopes in on select experiments state prediction comparison with visualisations of sample trajectories for a clear picture and context. Details on choices of experiment details such as training, hyperparamter choice, and NN architecture size/structure will be discussed in supplementary materials in the Appendix \ST{<- provided  the Appendix}. \ST{we should better to state here why these env are relevant, as we disccced in slack: diversity, stabilization , locomotion, diff body etc}.  \\

The comparable baselines for reference are: 
\begin{itemize}
  \item Feed-forward Deterministic Model, $f(s, a) \rightarrow s'$, \ST{it is not clear what 'f' mean} train with direct MSE loss on true state \ST{REF?}, we implement this ourselves \ST{<- can be omitted. "we implement this ourselves"  }
  \item Ensemble Deterministic Model, We Take the above Feed-Forward Model and spawn 5 instances and average output. $\frac{\sum_{i=0}^4 f_i(s,a)}{5} \rightarrow s'$
  \end{itemize}

We choose these baselines to represent the most comparable network to GEM. GEM and the baselines learn relationships from a feed forward multi layer perception, the crucial difference is what is being learned: direct state or Lie algebra coefficients. Ensembles provide a look into the effects of improved network architecture in prediction, we place the GEM architecture into an ensemble to show versatility. [REF Papers that use FF baseline, Ensembles] 
\ST{why do we show single and ensemble? any decision must have a reason. it is a technical paper being submitted ot the top conf.. any sentence should be justified/clear. }

Our experiments aim to answer three main questions:
\begin{center}
\begin{itemize}
    \item Does GEM achieve better long horizon prediction?
    \item Does GEM achieve higher performance in downstream tasks?
    \item Can GEM achieve higher rewards within fewer samples trained?
\end{itemize}
\end{center}
We answer the first question in Section 4 and the second two questions in Section 6.

\subsection{Long Horizon Prediction}
In long horizon prediction, our main goal is to compare the predictive power of GEM and baselines. Which will help answer our first main question. A strong model should be accurate, even in long horizon.\ST{what the diff between "accurate and secondly reliable". GOLDEN RULE: ALL WHAT IS UNNECESSARY GETS OUT OF THE PAPER}.  Having a model good at single step prediction only isn't useful for realistic application purposes. Many planners require models to be reliable for longer than one step to calculate optimal actions [REF PAPER FOR THIS]\ST{why? add refs for MBRL. }. We must evaluate the model not only on single step prediction, but on multiple step prediction to test its capabilities \ST{REFs, and we should put a hook for this statement}. 

For our main results, we set up experiments where models predict future states in a trajectory for up to 25 to 50 steps, which is a common planning horizon in RL [REF HERE]. \ST{as done where? why 25-50 is good? just put ref for any claim. don't assume reviewers know that 25-50 is reasonably hard/long horizon. help them to know that by reference. otherwise our choice is arbitrary. } Figure 2 (RESHAPE AND REFORM) represents a summary of our prediction results on all 9 tasks. 

We use relative error to provide generalized comparison over all environments. \ST{sounds as we average between pendulum and reacher} \ST{qualitatively MSE will be the same, but MSE is differentible and often used as a loss rather than abs}.\ST{ do we want to show how we cal it?}. For more details on experiment details, evaluation procedures, and numerical details visit appendix WRITE APPENDIX DETAILS. \\

GEM models, for both single and ensemble architectures, performs better in almost all tasks in state prediction when compared to the relevant baselines. We see the Baseline Single Model perform the worst in prediction for future state, followed by the Baseline Ensemble. The Baseline Ensemble matches the performance of the GEM Single model some of the time which shows the structural benefits of GEM when considering the Single Models have a fifth of the total parameters than the Ensemble systems. 

The experiment confirms our hypothesis on the benefits of including structural geometric priors into our model prediction \ST{model?}, GEM incorporates beneficial structural information that leads to better prediction in long horizon trajectories. The only place where a Baseline performed better than GEM was in the walker task where the ensemble baseline outperformed slightly the GEM single model, though the large advantage in architecture is not to be ignored. We did not run ensemble experiments for Ant and Humanoid due to the huge amount of time required to train ensemble models in extremely complex state tasks. Ant and Humanoid have up to 3x amount of parameters needed for prediction. [REF] \ST{do we explain the training loop, why is it so expensive?}Though in comparison of the single models we still see a decrease in static error over the baseline. In the section 4.2, we will go into more detail on absolute error comparison for select environments and look at renderings. 

\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.1]{./images/figure4}
    \caption{Overall Relative Error Comparisons on 9 Continuous Control Tasks, Averaged Over 5 Seeds except for Ant/Humanoid which are Averaged over 3 Seeds, Relative Error Computed by taking average per step mean squared error over 1, 5, 10, 25, and 50 (if applicable) step trajectory predictions and normalizing relative to maximum error. GEM Outperforms its comparative Baseline in long horizon prediction in all tasks.}
    \label{fig:}
\end{figure*}

\subsection{Detailed\ST{sounds as |error|, ABS} Comparison}
Here we will discuss detailed comparisons of experiments and visualizations of sample trajectories\ST{why do we want to show renders? added value? why bars are not enough?} to help show the evolution of the state prediction over time-step. The images will also give a glimpse on how GEMs belief compares to the baselines overtime. As mentioned above, only having strong single step prediction in a model is largely useless for application purposes [REF]\ST{it should be justified via REFs}. Most applications, such as MBRL, require models to remain robust for longer horizons \ST{why? we know the answer: even MBRL sucks if a model can predict in a single/short horizon. make a hook to our next experiments here }. These experiments will show the per step error of the environments to give a better idea of the performance \ST{performance and reliability: what the diff between these two, i mean not linguistically but for eh purpose of conveying our message to the readers. do we want the readers/reviewer start thinking what feature of our model is in charge for reliability and what is in charge for performance}. Figure 3 shows the results for Pendulum, Double Pendulum, Swimmer, Walker, Hopper, and Humanoid\ST{more concrete. many? which env? and again why we show them here} environments. These results aim to answer question one and provide us a closer look from the result in Figure 2. For more information on the experiments and the rest of the env plots, visit the appendix.\ST{indeed the details will be in appendix/supplementary. nobody will look at them. BUT WE MUST STATE CLEAR CUT WHY WE SHOW A PARTICULAR PLOT/RESULT. WHY IS THAT PLOT IMPORTANT TO THE READERS?}

\begin{figure*}[!h]
\centering
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/invpenabsolute_nox}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/walkerabsolute_nox}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/swimmerabsolute_nox}
\end{subfigure}
\hfill
\end{figure*}
\begin{figure*}[!h]
\centering
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/hopperabsolute_nox}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/invdoubpenabsolute_nox}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=0.1]{./images/humanoidabsolute_nox}
\end{subfigure}
\hfill
    \caption{Absolute Error Comparison for multiple  environments. Y axis is in absolute mean squared error per step for entire state prediction, except for Humanoid which is just in static error prediction. X axis is the same for each column. The same conclusion can be seen from before where GEM model outperforms generic in prediction on average for all tasks.}
\end{figure*}

The details results delve deeper into the results from Figure 2. \ST{here we just zoom into diff environments. we do not provide additional evidences for our hypothesis} We see similar low step predictive power between all models, but in the longer horizon prediction tasks GEM scales better than the baseline. \ST{where do we see that?}.

\subsection{Visualized Trajectories\ST{Generated Trajectories? i am not sure "Generated Trajectories" is the best here but Rendering is a bit jargon}}
To help provide visualization of the models evolution of belief give\ST{why capital?} in long horizon prediction, we provide samples from trajectories for multiple environments\ST{what do these images add to the readers to understand the power of our method?}. These images will aid in understanding the strengths and faults of each model to better asses why we see differences in error in the previous experiments.
In Figure $\#$ are samples of trajectories visualized to show evolution of model prediction.
While a sub sample, notice after many time steps GEM remains intact and reliable. The baseline's performance has largely degraded by step 30 and is unreliably for further steps.

\begin{figure*}[!h]
\centering
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/truth0}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/truth15}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/truth30}
\end{subfigure}
\hfill
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/truth45}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/truth0}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/truth15}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/truth30}
\end{subfigure}
\hfill
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/truth45}
\end{subfigure}
\hfill
\end{figure*}
\begin{figure*}[!h]
\centering
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/beliefone0}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/beliefone15}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/beliefone30}
\end{subfigure}
\hfill
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invpenimages/beliefone45}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/beliefone0}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/beliefone15}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/beliefone30}
\end{subfigure}
\hfill
\hfill
\begin{subfigure}[t]{0.225\textwidth}
    \includegraphics[scale=.2]{./images/invdoubpenimages/beliefone45}
\end{subfigure}
\hfill
\end{figure*}


.




==> sections/plotsOnly.tex <==
\input{sections/absErrorPlots}
\newpage
\newpage
\input{sections/relErrorPlots}
\newpage
\newpage
\input{sections/mbrPlots}
\newpage
\newpage
\input{sections/planningRewardCurves}
\newpage
\newpage
\input{sections/renderings}

==> sections/renderings_2column.tex <==
\begin{figure}[!h]
  \centering
  \begin{subfigure}[b]{0.2425\linewidth}
    \includegraphics[scale=.27575]{./images/invpenimages/truth0}
  \end{subfigure}
  \begin{subfigure}[b]{0.2425\linewidth}
    \includegraphics[scale=.27575]{./images/invpenimages/truth15}
  \end{subfigure}
  \begin{subfigure}[b]{0.2425\linewidth}
    \includegraphics[scale=.27575]{./images/invpenimages/truth30}
  \end{subfigure}
  \begin{subfigure}[b]{0.2425\linewidth}
    \includegraphics[scale=.27575]{./images/invpenimages/truth45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/belieftwo0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/belieftwo15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/belieftwo30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/belieftwo45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/beliefone0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/beliefone15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/beliefone30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invpenimages/beliefone45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/truth0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/truth15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/truth30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/truth45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/belieftwo0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/belieftwo15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/swimmerimages/belieftwo30}
  \end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/swimmerimages/belieftwo45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/swimmerimages/beliefone0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/swimmerimages/beliefone15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/swimmerimages/beliefone30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/swimmerimages/beliefone45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/truth0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/truth15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/truth30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/truth45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/belieftwo0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/belieftwo15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/belieftwo30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/belieftwo45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/beliefone0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/beliefone15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/beliefone30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/HopperImages/beliefone45}
\end{subfigure}
\end{figure}
\begin{figure}[!h]
  \centering
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/truth0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/truth15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/truth30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/truth45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/belieftwo0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/belieftwo15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/belieftwo30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/belieftwo45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/beliefone0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/beliefone15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/beliefone30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/reacherimages/beliefone45}
  \end{subfigure}
  \\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/truth0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/truth15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/truth30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/truth45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/belieftwo0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/belieftwo15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/belieftwo30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/belieftwo45}
\end{subfigure}
\\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/beliefone0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/beliefone15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/beliefone30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/WalkerImages/beliefone45}
\end{subfigure}
\\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/truth0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/truth15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/truth30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/truth45}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/belieftwo0}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/belieftwo15}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/belieftwo30}
  \end{subfigure}
  \begin{subfigure}[t]{0.2425\linewidth}
    \includegraphics[scale=.275]{./images/invdoubpenimages/belieftwo45}
  \end{subfigure}
  \\
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/invdoubpenimages/beliefone0}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/invdoubpenimages/beliefone15}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/invdoubpenimages/beliefone30}
\end{subfigure}
\begin{subfigure}[t]{0.2425\linewidth}
  \includegraphics[scale=.275]{./images/invdoubpenimages/beliefone45}
\end{subfigure}
\end{figure}


==> sections/scheme1.tex <==
% \tikzset{fontscale/.style = {font=\relsize{#1}}}
% \usetikzlibrary{patterns}
% https://www.dumas.io/teaching/2017/fall/math549/
\begin{figure}[t]
% \begin{center}
\begin{tikzpicture}[scale=.5, transform shape, every node/.style={thick,circle,inner sep=0pt}]

% \node[inner sep=0pt] (humanoid) at (1.2,0.775) {\includegraphics[scale=0.14]{./images/humanoid_}};
\node[inner sep=0pt] (humanoid) at (1.2,0.775) {\includegraphics[scale=0.34]{./images/walkerTrue_}};
    
\node[inner sep=0pt] (manifold) at (1.2,3.3) {\includegraphics[scale=0.25]{./images/manifold}};

\node[inner sep=0pt, text width=2.5cm,text centered, rectangle, opacity=1.0, draw,dashed, rounded corners, minimum size=1.7cm] (algebra) at (1.2,5.3) {Lie Algebra: vector space  with a basis};


\node[circle, fill=Green!60, minimum size=1cm] (a3) at (6, 0)  {$\mathbf{a_{t-1}}$};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=2] (a2) at (3.7, -0.2)  {MDP};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=4] (g1) at (3.5, 1.7*1.65)  {${\LARGE\mathcal{G}}$};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=4] (ap12) at (3.5, 3.0*1.65)  {${\LARGE\mathfrak{g}}$};

\node[circle, fill=Green!60, minimum size=1cm] (a4) at (8, 0)  {$\mathbf{a_{t}}$};
\node[rectangle, fill=Red!40, minimum size=1cm] (ap3) at (6, 3.35*1.65)  {$\;\;\;\mathbf{\hat{g}_{t-1}}\;\;\;$};
\node[rectangle, fill=Red!40, minimum size=1cm] (ap4) at (8, 3.35*1.65)  {$\;\;\;\;\;\mathbf{\hat{g}_{t}}\;\;\;\;\;$};
\node[circle,  opacity=1.0, minimum size=1cm] (g2) at (3, 2.2*1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (ap2) at (3, 3.35*1.65) {};
\node[circle, opacity=1.0, minimum size=1cm] (x2) at (3, 1.65) {};
\node[circle, fill=Green!60, minimum size=1cm] (x3) at (5, 1.65) {$\mathbf{s_{t-1}}$};
\node[circle, fill=Green!60, minimum size=1cm] (x4) at (7, 1.65) {$\mathbf{s_t}$};
\node[circle, fill=Green!60, minimum size=1cm] (x5) at (9, 1.65) {$\mathbf{s_{t+1}}$};
\node[circle,  opacity=1.0, minimum size=1cm] (x6) at (11, 1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (g6) at (11, 2.1*1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (al6) at (11, 3.35*.65) {};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.2cm] (g3) at (5, 2.1*1.65) {$\mathbf{G_{t-1}}$};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.25cm] (g4) at (7, 2.1*1.65) {$\mathbf{G_t}$};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.2cm] (g5) at (9, 2.1*1.65) {$\mathbf{G_{t+1}}$};
\foreach \from/\to in {x3/a3, x3/x4, a3/x4, x4/x5, x4/a4, a4/x5,x2/x3,x5/x6}
\draw [->] (\from) -- (\to);
\foreach \from/\to in {x3/g3,x4/g4,x5/g5}
\draw [->] (\from) -- (\to);
\foreach \from/\to in {ap3/g4,ap4/g5,g3/ap3,g4/ap4,g3/g4,g4/g5}
\draw [->] (\from) -- (\to);
\begin{pgfonlayer}{background}
        \path (x2.west |- x2.north)+(+0.5,+0.1) node (a) {};
        \path (x2.east -| x2.east)+(+7.5,-2.25) node (c) {};
        \path[fill=gray!5,pattern=crosshatch dots, fill opacity=0.5,rounded corners, draw=black!10, dashed] (a) rectangle (c);           
\end{pgfonlayer}
\begin{pgfonlayer}{background}
        \path (g2.west |- g2.north)+(+0.5,+0.15) node (a) {};
        \path (g2.east -| g2.east)+(+7.5,-1.25) node (c) {};
        \path[fill=gray!10,pattern=crosshatch, fill opacity=0.2,rounded corners, draw=black!10,dashed] (a) rectangle (c);           
\end{pgfonlayer}
\begin{pgfonlayer}{background}
        \path (ap2.west |- ap2.north)+(+0.5,+0.15) node (a) {};
        \path (ap2.east -| ap2.east)+(+7.5,-1.1) node (c) {};
        \path[fill=gray!15,pattern=grid,fill opacity=0.2, rounded corners, draw=black!10,dashed] (a) rectangle (c);           
\end{pgfonlayer}
\end{tikzpicture}
% \end{center}
\caption{MDP, $\mathcal{G}$ and $\mathfrak{g}$ denote Markov Decision Process, Lie Group (manifold, $\mathcal{M}$), and Lie Algebra, respectively. $(s_t\in\mathcal{S}, a_t\in\mathcal{A})$, $G_t\in\mathcal{G}$, and $g_{t}\in\mathfrak{g}$, are observable state and action, a constructed Lie group element, and an estimated Lie algebra element, respectively. The original dynamics, $s_{t+1}=f(s_t, a_t)$ is learnt through the dynamics on the Lie group, $G_{t+1}=\exp(\hat{g}_t)\circ G_t$, where $\hat{g} = \sum_i \hat{\alpha}_{{\theta}_{i}}\cdot E_{i}$ with $E=\{E_i\}_i$ and $\alpha_{{\theta}_{i}}$ is a Lie algebra basis, and the Lie algebra coefficients, parameterized by $\theta$, respectively.} \label{fig:scheme1}
\end{figure}



==> sections/scheme1_tikz.tex <==
\begin{tikzpicture}[scale=.5, transform shape, every node/.style={thick,circle,inner sep=0pt}]

% \node[inner sep=0pt] (humanoid) at (1.2,0.775) {\includegraphics[scale=0.14]{./images/humanoid_}};
\node[inner sep=0pt] (humanoid) at (1.2,0.775) {\includegraphics[scale=0.375]{./images/walkerTrue_}};
    
\node[inner sep=0pt] (manifold) at (1.2,3.3) {\includegraphics[scale=0.25]{./images/manifold}};

\node[inner sep=0pt, text width=2.5cm,text centered, rectangle, opacity=1.0, draw,dashed, rounded corners, minimum size=1.7cm] (algebra) at (1.2,5.3) {Lie Algebra: vector space  with a basis};


\node[circle, fill=Green!60, minimum size=1cm] (a3) at (6, 0)  {$\mathbf{a_{t-1}}$};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=2] (a2) at (3.7, -0.2)  {MDP};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=4] (g1) at (3.5, 1.7*1.65)  {${\LARGE\mathcal{G}}$};
\node[circle,  opacity=1.0,minimum size=1cm,fontscale=4] (ap12) at (3.5, 3.0*1.65)  {${\LARGE\mathfrak{g}}$};

\node[circle, fill=Green!60, minimum size=1cm] (a4) at (8, 0)  {$\mathbf{a_{t}}$};
\node[rectangle, fill=Red!40, minimum size=1cm] (ap3) at (6, 3.35*1.65)  {$\;\;\;\mathbf{\hat{g}_{t-1}}\;\;\;$};
\node[rectangle, fill=Red!40, minimum size=1cm] (ap4) at (8, 3.35*1.65)  {$\;\;\;\;\;\mathbf{\hat{g}_{t}}\;\;\;\;\;$};
\node[circle,  opacity=1.0, minimum size=1cm] (g2) at (3, 2.2*1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (ap2) at (3, 3.35*1.65) {};
\node[circle, opacity=1.0, minimum size=1cm] (x2) at (3, 1.65) {};
\node[circle, fill=Green!60, minimum size=1cm] (x3) at (5, 1.65) {$\mathbf{s_{t-1}}$};
\node[circle, fill=Green!60, minimum size=1cm] (x4) at (7, 1.65) {$\mathbf{s_t}$};
\node[circle, fill=Green!60, minimum size=1cm] (x5) at (9, 1.65) {$\mathbf{s_{t+1}}$};
\node[circle,  opacity=1.0, minimum size=1cm] (x6) at (11, 1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (g6) at (11, 2.1*1.65) {};
\node[circle,  opacity=1.0, minimum size=1cm] (al6) at (11, 3.35*.65) {};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.2cm] (g3) at (5, 2.1*1.65) {$\mathbf{G_{t-1}}$};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.25cm] (g4) at (7, 2.1*1.65) {$\mathbf{G_t}$};
\node[regular polygon,regular polygon sides=9, fill=NavyBlue!60, minimum size=1.2cm] (g5) at (9, 2.1*1.65) {$\mathbf{G_{t+1}}$};
\foreach \from/\to in {x3/a3, x3/x4, a3/x4, x4/x5, x4/a4, a4/x5,x2/x3,x5/x6}
\draw [->] (\from) -- (\to);
\foreach \from/\to in {x3/g3,x4/g4,x5/g5}
\draw [->] (\from) -- (\to);
\foreach \from/\to in {ap3/g4,ap4/g5,g3/ap3,g4/ap4,g3/g4,g4/g5}
\draw [->] (\from) -- (\to);
\begin{pgfonlayer}{background}
        \path (x2.west |- x2.north)+(+0.5,+0.1) node (a) {};
        \path (x2.east -| x2.east)+(+7.5,-2.25) node (c) {};
        \path[fill=gray!5,pattern=crosshatch dots, fill opacity=0.5,rounded corners, draw=black!10, dashed] (a) rectangle (c);           
\end{pgfonlayer}
\begin{pgfonlayer}{background}
        \path (g2.west |- g2.north)+(+0.5,+0.15) node (a) {};
        \path (g2.east -| g2.east)+(+7.5,-1.25) node (c) {};
        \path[fill=gray!10,pattern=crosshatch, fill opacity=0.2,rounded corners, draw=black!10,dashed] (a) rectangle (c);           
\end{pgfonlayer}
\begin{pgfonlayer}{background}
        \path (ap2.west |- ap2.north)+(+0.5,+0.15) node (a) {};
        \path (ap2.east -| ap2.east)+(+7.5,-1.1) node (c) {};
        \path[fill=gray!15,pattern=grid,fill opacity=0.2, rounded corners, draw=black!10,dashed] (a) rectangle (c);           
\end{pgfonlayer}
\end{tikzpicture}

==> sections/tables.tex <==
\usepackage{bigstrut}

\section{Tables}
\subsection{Demo}
\begin{tabular}{c c c c}
\hline
{} &         \text{Lie Small Model} &         \text{Lie Medium Model} &         \text{Lie Large Model}\\
\hline
\shortstack{\textb{Inverted Pendulum 1-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.00456 \pm 0.00010 \\ \textit{Static:} 0.00061 \pm 0.00001 \\ \textit{Dynamic:} 0.00398 \pm 0.00009} &  \shortstack{\textit{Total:} 0.00760 \pm 0.00014  \\ \textit{Static:} 0.00042 \pm 0.00001 \\ \textit{Dynamic:} 0.00718 \pm 0.00014} &  \shortstack{\textit{Total:} 0.01228 \pm 0.00029  \\ \textit{Static:} 0.00039 \pm 0.00002 \\ \textit{Dynamic:} 0.01189 \pm 0.00028} \\
\hline
\shortstack{\textb{Inverted Pendulum 5-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.02160 \pm 0.00021 \\ \textit{Static:} 0.00186 \pm 0.00004 \\ \textit{Dynamic:} 0.01974 \pm 0.00019} &  \shortstack{\textit{Total:} 0.02304 \pm 0.00060  \\ \textit{Static:} 0.00214 \pm 0.00004 \\ \textit{Dynamic:} 0.02090 \pm 0.00057} &  \shortstack{\textit{Total:} 0.03813 \pm 0.00090  \\ \textit{Static:} 0.00202 \pm 0.00007 \\ \textit{Dynamic:} 0.03611 \pm 0.00090}  \\
\hline
\shortstack{\textb{Inverted Pendulum 10-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.06167 \pm 0.00056 \\ \textit{Static:} 0.00706 \pm 0.00006 \\ \textit{Dynamic:} 0.05461 \pm 0.00028} &  \shortstack{\textit{Total:} 0.05158 \pm 0.00031 \\ \textit{Static:} 0.00529 \pm 0.00007 \\ \textit{Dynamic:} 0.04629 +-  0.00050} &  \shortstack{\textit{Total:} 0.048341 +- 0.00085 \\ \textit{Static:} 0.04304 +- 0.00084 \\ \textit{Dynamic:} 0.05461 +- 0.00028}  \\
\hline
\shortstack{\textb{Inverted Pendulum 25-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.28671 +- 0.00307 \\ \textit{Static:} 0.05372 +- 0.00055 \\ \textit{Dynamic:} 0.23299 +- 0.00253} &  \shortstack{\textit{Total:} 0.40593 +- 0.00467 \\ \textit{Static:} 0.07133 +- 0.00085 \\ \textit{Dynamic:} 0.33460 +-  0.003818} &  \shortstack{\textit{Total:} 0.40690 +- 0.00875 \\ \textit{Static:} 0.07452 +- 0.00168 \\ \textit{Dynamic:} 0.33238 +- 0.00708}  \\
\hline
\shortstack{{Inverted Pendulum 50-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 2.8899 +- 0.08694 \\ \textit{Static:} 0.76304 +- 0.01664 \\ \textit{Dynamic:} 2.12683 +- 0.07050} &  \shortstack{\textit{Total:} 3.74402 +- 0.07972 \\ \textit{Static:} 0.84065 +- 0.01011 \\ \textit{Dynamic:} 2.90337 +-  0.07107} &  \shortstack{\textit{Total:} 4.41028 +- 0.04637 \\ \textit{Static:} 0.90914 +- 0.01019 \\ \textit{Dynamic:} 3.50115 +- 0.03638} 
\end{tabular}

\subsection{Your Table}

\begin{tabular}{c c c c}
\hline
{} &         \text{Generic Small Model} &         \text{Generic Medium Model} &         \text{Generic Large Model}\\
\hline
\shortstack{\textb{Inverted Pendulum 1-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.01820 \pm 0.00013 \\ \textit{Static:} 0.00505 \pm 0.00006 \\ \textit{Dynamic:} 0.01042 \pm 0.00012} &  \shortstack{\textit{Total:} 0.02461 \pm 0.00018  \\ \textit{Static:} 0.00432 \pm 0.00002 \\ \textit{Dynamic:} 0.01708 \pm 0.00016} &  \shortstack{\textit{Total:} 0.02129 \pm 0.00042  \\ \textit{Static:} 0.00608 \pm 0.00021 \\ \textit{Dynamic:} 0.01219 \pm 0.00027} \\
\hline
\shortstack{\textb{Inverted Pendulum 5-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.07222 \pm 0.00013 \\ \textit{Static:} 0.01824 \pm 0.00003 \\ \textit{Dynamic:} 0.04994 \pm 0.00011} &  \shortstack{\textit{Total:} 0.07905 \pm 0.00069  \\ \textit{Static:} 0.01452 \pm 0.00018 \\ \textit{Dynamic:} 0.06139 \pm 0.00058} &  \shortstack{\textit{Total:} 0.08146 \pm 0.00152  \\ \textit{Static:} 0.03312 \pm 0.00056 \\ \textit{Dynamic:} 0.04567 \pm 0.00111}  \\
\hline
\shortstack{\textb{Inverted Pendulum 10-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.12948 \pm 0.00051 \\ \textit{Static:} 0.03228 \pm 0.00010 \\ \textit{Dynamic:} 0.09300 \pm 0.00044} &  \shortstack{\textit{Total:} 0.16450 \pm 0.00127 \\ \textit{Static:} 0.03350 \pm 0.00033 \\ \textit{Dynamic:} 0.12771 +-  0.00100} &  \shortstack{\textit{Total:} 0.19850 +- 0.00193 \\ \textit{Static:} 0.03648 +- 0.00102 \\ \textit{Dynamic:} 0.16105 +- 0.00267}  \\
\hline
\shortstack{\textb{Inverted Pendulum 25-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 0.90972 +- 0.00640 \\ \textit{Static:} 0.17669 +- 0.00118 \\ \textit{Dynamic:} 0.72476 +- 0.00520} &  \shortstack{\textit{Total:} 1.65210 +- 0.01064 \\ \textit{Static:} 0.39979 +- 0.00244 \\ \textit{Dynamic:} 1.20853 +-  0.00800} &  \shortstack{\textit{Total:} 0.85274 +- 0.00806 \\ \textit{Static:} 0.13769 +- 0.00134 \\ \textit{Dynamic:} 0.71288 +- 0.00714}  \\
\hline
\shortstack{{Inverted Pendulum 50-Step} \\ {} \\ {}} &  \shortstack{\textit{Total:} 21.63696 +- 0.06196 \\ \textit{Static:} 4.74914 +- 0.01373 \\ \textit{Dynamic:} 15.29290 +- 0.043143} &  \shortstack{\textit{Total:} 497.25837 +- 18.5497 \\ \textit{Static:} 199.53331 +- 5.61142 \\ \textit{Dynamic:} 248.53911 +-  11.37884} &  \shortstack{\textit{Total:} 2.13719 +- 0.00980 \\ \textit{Static:} 0.21421 +- 0.00136 \\ \textit{Dynamic:} 1.92224 +- 0.00926} 
\end{tabular}




